On the satisfiability of random $3$-SAT formulas with $k$-wise independent clauses

The problem of identifying the satisfiability threshold of random $3$-SAT formulas has received a lot of attention during the last decades and has inspired the study of other threshold phenomena in random combinatorial structures. The classical assumption in this line of research is that, for a given set of $n$ Boolean variables, each clause is drawn uniformly at random among all sets of three literals from these variables, independently from other clauses. Here, we keep the uniform distribution of each clause, but deviate significantly from the independence assumption and consider richer families of probability distributions. For integer parameters $n$, $m$, and $k$, we denote by $\DistFamily_k(n,m)$ the family of probability distributions that produce formulas with $m$ clauses, each selected uniformly at random from all sets of three literals from the $n$ variables, so that the clauses are $k$-wise independent. Our aim is to make general statements about the satisfiability or unsatisfiability of formulas produced by distributions in $\DistFamily_k(n,m)$ for different values of the parameters $n$, $m$, and $k$.

==> largesat.tex <==



==> related.tex <==
\begin{enumerate}
    \item Phase transition in random $k$-SAT
    \begin{itemize}
        \item Uniform distribution with independent clauses
        \item Non-uniform distributions.
    \end{itemize}
    \item Specific results about $3$-SAT
    \begin{enumerate}
        \item Phase transition: Theory papers, practice $+$ numerical experiments.
        \item Computational questions of proving unsatisfiability:
        \begin{itemize}
            \item Friedman, Goerdt, and Krivelevich~\cite{FriedmanGK05} give a polynomial time algorithm via spectral techniques that refutes a random SAT forumal with $m=n^{3/2+\eps}$.
            \item Feige and Ofek~\cite{FeigeO07} show how to certify unsatisfiability in polytime for most random SAT formulas, for $m=c\cdot n^{3/2}$. Their proof relies on the $3$XOR principle that search for pairs of $3$CNF clauses with two shared literals and treats them as XOR clauses. Our proofs share similar features in (a) constructing $3$-clause independent distribution   based on XOR literals with $m=\Theta(n^3)$ clauses and constant SAT probability, and (b) in studying  bipartite graph between single literals and literal pairs, i.e., looking at the intersection of size $2$ between clause literals. It has also been mentioned in~\cite{FeigeO07} that for $m=O(n^2)$ it is easy to find a refutation: by considering all clauses ($m_1=c\cdot n$) with a fixed variable $X_1$ and refuting two induced random $2$SAT instances. It is interesting to note that this approach critically relies on mutual independence and does not seem to work well for $4$-clause independent distributions.
            \item Chvatal and Szemeredi~\cite{ChvatalS88} showed that a random $3$CNF formula with $m=\Theta(n)$ clauses almost surely admits only an exponential size for the resolution proof.
            \item Ben-Sasson and Wigderson~\cite{BenSassonW01} showed that even
            for $m=O(n^{3/2-\eps})$ a random $3$CNF formula likely has exponential 
            size of the resolution proof. 

        \end{itemize}        
        \item Algorithms for finding satisfiable assignments:
        \begin{itemize}
            \item Krivelevich and Vilenchik~\cite{KrivelevichV06} give an algorithm with expected polynomial running time that finds solution in a random $m=c\cdot n$ $3$SAT instance with planted solution for sufficiently large $c$. 
            \item Various heuristic approaches for random formulas with $m=c\cdot n$ clauses, where $c$ is smaller than the conjectured satisfiability threshold, are shown to find satisfying assignments with high probability. \nick{A useful summary at:}\verb+https://www.math.cmu.edu/~adf/research/rand-sat-algs.pdf+
        \end{itemize}
    \end{enumerate}
    \item Guarantees for $k$-wise independence. 
    \begin{enumerate}
        \item Recent work on Bayesian optimization with $k$-wise independent prior distribution given by the marginals.
        \item Alon and Nussboim~\cite{AlonN08} study the required $k$ for various properties to hold in random $k$-wise independent graphs.
        \item \cite{BenjaminiGP12} examine the required degree of independence $k$ such that given monotone boolean functions such as AND, Majority, Tribes, and Percolation give similar results on any $k$-wise independent distribution of inputs as on mutually independent distribution.  
    \end{enumerate}
\end{enumerate}



\Zhile{Here are some paper related to the transition phase of random SAT or just random SAT.}



\cite{CKT1991,MSL1992} suggest the transition phase in numerical experiments.

\cite{CR1992} proves the satisfiability threshold is $1$ for random $2$-SAT.

\cite{BBCKW2001} determines the window of transition as $[n-\Theta(n^{1/3}), n+\Theta(n^{1/3})]$.

\cite{DSS2022} closes the conjecture for random $k$-SAT with sufficiently large $k$.


The conjecture for $k\geq 3$ is still open. On the lower bound, \cite{CR1992} first shows it is at least $2/3$. \cite{BFU1993} improves it to $1.63$. It is later improved to $3.003$ by \cite{FS1996}. \cite{Achlioptas2000} improves it to $3.145$, which is the best results until now. On the upper bound, it is first shown to be at most $5.191$ by \cite{FP1983}. There is a line of work \cite{MV95, KMPS95, DB97, KKKS98, JSV00, DBM2000}. The state-of-the-art is $4.506$ by \cite{DBM2000}.

The current lower bound:\cite{HS03, KKL06, DKMP09}; The estimation by cavity method:\cite{MMZ06} \nick{The current lower and upper bounds for $3$-SAT have been improved. From Non Uniform random SAT ICALP paper: 
$3.52\le r_3\le 4.4898$ [19, 24, 25] and numerical estimates using the cavity method from statistical mechanics [29] suggest that
$r_3\approx  4.26$.}

\cite{FKRRS2017, FR2018, FR2019, OB2019} study the satisfiability in non-uniform random $k$-SAT.

\cite{HJ2012} solves planted-XOR-$k$-SAT (the way our constructions plant solution) efficiently.
